Privacy Risks in Time Series Forecasting: User- and Record-Level Membership Inference

Membership inference attacks (MIAs) aim to determine whether specific data were used to train a model. While extensively studied on classification models, their impact on time series forecasting remains largely unexplored. We address this gap by introducing two new attacks: (i) an adaptation of multivariate LiRA, a state-of-the-art MIA originally developed for classification models, to the time-series forecasting setting, and (ii) a novel end-to-end learning approach called Deep Time Series (DTS) attack. We benchmark these methods against adapted versions of other leading attacks from the classification setting. We evaluate all attacks in realistic settings on the TUH-EEG and ELD datasets, targeting two strong forecasting architectures, LSTM and the state-of-the-art N-HiTS, under both record- and user-level threat models. Our results show that forecasting models are vulnerable, with user-level attacks often achieving perfect detection. The proposed methods achieve the strongest performance in several settings, establishing new baselines for privacy risk assessment in time series forecasting. Furthermore, vulnerability increases with longer prediction horizons and smaller training populations, echoing trends observed in large language models.

==> Results_includes/attack_ROC_offline_fig.tex <==

\pgfplotscreateplotcyclelist{mycolors}{
    {blue, mark=none},
    {red, mark=none},
    {green!60!black, mark=none},
    {orange, mark=none},
    {purple, mark=none},
    {brown, mark=none},
    {cyan!60!black, mark=none},
}



\begin{figure*}[ht]
\centering

% Row1: RMIA
\input{offline_ROCs_rows/RMIA}

% Row2: LiRA
\input{offline_ROCs_rows/LiRA}

% Row3: Multi-LiRA
 \input{offline_ROCs_rows/Multi-LiRA}

% Row4: DTS
 \input{offline_ROCs_rows/DTS}

\par\vspace{1em}


\caption{ROC curves with logarithmic scales (TPR on the y-axis and FPR on the x-axis) for four membership inference attacks: RMIA, LiRA, Multi-Signal LiRA, and DTS, arranged in columns. Rows correspond to dataset–architecture pairs: EEG–LSTM, EEG–N-HiTS, ELD–LSTM, and ELD–N-HiTS. 
All results are for the \textbf{offline} setting. Within each subplot, curves correspond to individual attack signals for LiRA, and RMIA, all combined signals for Multi-Signal LiRA, and different classifier architectures for DTS. Each curve represents the mean over five independent runs.
}
\label{fig:roc_offline}
\end{figure*}















==> Results_includes/attack_ROC_online_fig.tex <==
\pgfplotscreateplotcyclelist{mycolors}{
    {blue, mark=none},
    {red, mark=none},
    {green!60!black, mark=none},
    {orange, mark=none},
    {purple, mark=none},
    {brown, mark=none},
    {cyan!60!black, mark=none},
}

\begin{figure*}[ht]
\centering

% Row1: Ensemble
\input{online_ROCs_rows/Ensemble}

% Row2: RMIA
\input{online_ROCs_rows/RMIA}

% Row3: LiRA
\input{online_ROCs_rows/LiRA}

% Row4: Multi-LiRA
 \input{online_ROCs_rows/Multi-LiRA}

% Row5: DTS
 \input{online_ROCs_rows/DTS}

\par\vspace{1em}


\caption{ROC curves with logarithmic scales (TPR on the y-axis and FPR on the x-axis) for five membership inference attacks: Ensemble, RMIA, LiRA, Multi-Signal LiRA, and DTS, arranged in rows. Columns correspond to dataset–architecture pairs: EEG–LSTM, EEG–N-HiTS, ELD–LSTM, and ELD–N-HiTS. All results are for the \textbf{online} setting, with the Ensemble attack evaluated in audit mode. Within each subplot, curves correspond to individual attack signals for LiRA, RMIA, and Ensemble, all combined signals for Multi-Signal LiRA, and different classifier architectures for DTS. Each curve represents the mean over five independent runs.}
\label{fig:roc_online}
\end{figure*}















==> Results_includes/offline_ROCs_rows/DTS.tex <==
\pgfplotsset{
  every axis/.append style={
    label style={font=\normalsize},
    tick label style={font=\normalsize},
    legend style={font=\normalsize},
  }
}

% ------------ Subfigure 1 ------------
\begin{subfigure}[t]{0.22\textwidth}
\centering
\begin{tikzpicture}[scale=0.5]
  \begin{axis}[
    xmode=log, ymode=log,
    log basis y = 10,
    each nth point={10},
    xmin=1e-4, ymin=1e-4, xmax=1, ymax=1,
    xlabel={FPR}, ylabel={TPR (DTS)},
    grid=major,
    legend pos={south east},
    legend style={/tikz/every node/.append style={anchor=west}},
    every axis plot/.append style={line width=1pt},
    cycle list name=mycolors,
  ]
    
    \addplot [gray, dashed, domain=1e-4:1, samples=100, forget plot] {x};


    \addplot+[
    mark=none]
    table[x=fpr, y=tpr, col sep=comma] {data/EEG/DTS/LSTM-offline/total/roc_InceptionTimeS.csv};
    \addlegendentry{InceptionTime}
    
    \addplot+[mark=none]
    \addlegendentry{LSTM}
    
    
  \end{axis}
\end{tikzpicture}
% % \caption{Model 1}
\end{subfigure}
% ------------ Subfigure 2 ------------
\begin{subfigure}[t]{0.22\textwidth}
\centering
\begin{tikzpicture}[scale=0.5]
  \begin{axis}[
    xmode=log, ymode=log,
    xmin=1e-4, ymin=1e-4, xmax=1, ymax=1,
    xlabel={FPR}, ylabel={},
    grid=major,
    each nth point={10},
    legend pos={south east},
    legend style={/tikz/every node/.append style={anchor=west}},
    every axis plot/.append style={line width=1pt},
    cycle list name=mycolors,
  ]
  \addplot [gray, dashed, domain=1e-4:1, samples=100, forget plot] {x};
  
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/DTS/NHiTS-offline/total/roc_InceptionTimeS.csv};
    \addlegendentry{InceptionTime}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/DTS/NHiTS-offline/total/roc_LSTM.csv};
    \addlegendentry{LSTM}
    
  \end{axis}
\end{tikzpicture}
% \caption{Model 2}
\end{subfigure}
% ------------ Subfigure 3 ------------
\begin{subfigure}[t]{0.22\textwidth}
\centering
\begin{tikzpicture}[scale=0.5]
  \begin{axis}[
    xmode=log, ymode=log,
    xmin=1e-4, ymin=1e-4, xmax=1, ymax=1,
    xlabel={FPR}, ylabel={},
    grid=major,
    each nth point={10},
    legend pos={south east},
    legend style={/tikz/every node/.append style={anchor=west}},
    every axis plot/.append style={line width=1pt},
    cycle list name=mycolors,
  ]
  \addplot [gray, dashed, domain=1e-4:1, samples=100, forget plot] {x};
  
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/DTS/LSTM-offline/total/roc_InceptionTimeS.csv};
    \addlegendentry{InceptionTime}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/DTS/LSTM-offline/total/roc_LSTM.csv};
    \addlegendentry{LSTM}
    
  \end{axis}
\end{tikzpicture}
% \caption{Model 1}
\end{subfigure}
% ------------ Subfigure 4 ------------
\begin{subfigure}[t]{0.22\textwidth}
\centering
\begin{tikzpicture}[scale=0.5]
  \begin{axis}[
    xmode=log, ymode=log,
    xmin=1e-4, ymin=1e-4, xmax=1, ymax=1,
    xlabel={FPR}, ylabel={},
    grid=major,
    each nth point={10},
    legend pos={south east},
    legend style={/tikz/every node/.append style={anchor=west}},
    every axis plot/.append style={line width=1pt},
    cycle list name=mycolors,
  ]
  \addplot [gray, dashed, domain=1e-4:1, samples=100, forget plot] {x};
  
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/DTS/NHiTS-offline/total/roc_InceptionTimeS.csv};
    \addlegendentry{InceptionTime}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/DTS/NHiTS-offline/total/roc_LSTM.csv};
    \addlegendentry{LSTM}

  \end{axis}
\end{tikzpicture}
% \caption{Model 1}
\end{subfigure}


==> Results_includes/offline_ROCs_rows/LiRA.tex <==
\pgfplotsset{
  every axis/.append style={
    label style={font=\normalsize},
    tick label style={font=\normalsize},
    legend style={font=\normalsize},
  }
}

% ------------ Subfigure 1 ------------
\begin{subfigure}[t]{0.22\textwidth}
\centering
\begin{tikzpicture}[scale=0.5]
  \begin{axis}[
    xmode=log, ymode=log,
    log basis y = 10,
    each nth point={10},
    xmin=1e-4, ymin=1e-4, xmax=1, ymax=1,
    xlabel={FPR}, ylabel={TPR (LiRA)},
    grid=major,
    legend pos={south east},
    legend style={/tikz/every node/.append style={anchor=west}},
    every axis plot/.append style={line width=1pt},
    cycle list name=mycolors,
     title={TUH-EEG, LSTM},
  ]
    
    \addplot [gray, dashed, domain=1e-4:1, samples=100, forget plot] {x};


    \addplot+[
    mark=none]
    table[x=fpr, y=tpr, col sep=comma] {data/EEG/LiRA/LSTM-offline/total/roc_MAELoss.csv};
    \addlegendentry{MAE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/LiRA/LSTM-offline/total/roc_MSELoss.csv};
    \addlegendentry{MSE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/LiRA/LSTM-offline/total/roc_SeasonalityLoss.csv};
    \addlegendentry{Seasonality}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/LiRA/LSTM-offline/total/roc_SMAPELoss.csv};
    \addlegendentry{SMAPE Loss}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/LiRA/LSTM-offline/total/roc_RescaledSMAPELoss.csv};
    \addlegendentry{Rescaled SMAPE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/LiRA/LSTM-offline/total/roc_TrendLoss.csv};
    \addlegendentry{Trend}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/LiRA/LSTM-offline/total/roc_TS2VecLoss.csv};
    \addlegendentry{TS2Vec}
    
  \end{axis}
\end{tikzpicture}
% \caption{Model 1}
\end{subfigure}
% ------------ Subfigure 2 ------------
\begin{subfigure}[t]{0.22\textwidth}
\centering
\begin{tikzpicture}[scale=0.5]
  \begin{axis}[
    xmode=log, ymode=log,
    xmin=1e-4, ymin=1e-4, xmax=1, ymax=1,
    xlabel={FPR}, ylabel={},
    grid=major,
    each nth point={10},
    legend pos={south east},
    legend style={/tikz/every node/.append style={anchor=west}},
    every axis plot/.append style={line width=1pt},
    cycle list name=mycolors,
     title={TUH-EEG, N-HiTS},
  ]
  \addplot [gray, dashed, domain=1e-4:1, samples=100, forget plot] {x};
  
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/LiRA/NHiTS-offline/total/roc_MAELoss.csv};
    \addlegendentry{MAE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/LiRA/NHiTS-offline/total/roc_MSELoss.csv};
    \addlegendentry{MSE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/LiRA/NHiTS-offline/total/roc_SeasonalityLoss.csv};
    \addlegendentry{Seasonality}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/LiRA/NHiTS-offline/total/roc_SMAPELoss.csv};
    \addlegendentry{SMAPE Loss}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/LiRA/NHiTS-offline/total/roc_RescaledSMAPELoss.csv};
    \addlegendentry{Rescaled SMAPE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/LiRA/NHiTS-offline/total/roc_TrendLoss.csv};
    \addlegendentry{Trend}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/LiRA/NHiTS-offline/total/roc_TS2VecLoss.csv};
    \addlegendentry{TS2Vec}
  \end{axis}
\end{tikzpicture}
% \caption{Model 2}
\end{subfigure}
% ------------ Subfigure 3 ------------
\begin{subfigure}[t]{0.22\textwidth}
\centering
\begin{tikzpicture}[scale=0.5]
  \begin{axis}[
    xmode=log, ymode=log,
    xmin=1e-4, ymin=1e-4, xmax=1, ymax=1,
    xlabel={FPR}, ylabel={},
    grid=major,
    each nth point={10},
    legend pos={south east},
    legend style={/tikz/every node/.append style={anchor=west}},
    every axis plot/.append style={line width=1pt},
    cycle list name=mycolors,
     title={ELD, LSTM},
  ]
  \addplot [gray, dashed, domain=1e-4:1, samples=100, forget plot] {x};
  
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/LiRA/LSTM-offline/total/roc_MAELoss.csv};
    \addlegendentry{MAE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/LiRA/LSTM-offline/total/roc_MSELoss.csv};
    \addlegendentry{MSE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/LiRA/LSTM-offline/total/roc_SeasonalityLoss.csv};
    \addlegendentry{Seasonality}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/LiRA/LSTM-offline/total/roc_SMAPELoss.csv};
    \addlegendentry{SMAPE Loss}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/LiRA/LSTM-offline/total/roc_RescaledSMAPELoss.csv};
    \addlegendentry{Rescaled SMAPE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/LiRA/LSTM-offline/total/roc_TrendLoss.csv};
    \addlegendentry{Trend}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/LiRA/LSTM-offline/total/roc_TS2VecLoss.csv};
    \addlegendentry{TS2Vec}
  \end{axis}
\end{tikzpicture}
% \caption{Model 1}
\end{subfigure}
% ------------ Subfigure 4 ------------
\begin{subfigure}[t]{0.22\textwidth}
\centering
\begin{tikzpicture}[scale=0.5]
  \begin{axis}[
    xmode=log, ymode=log,
    xmin=1e-4, ymin=1e-4, xmax=1, ymax=1,
    xlabel={FPR}, ylabel={},
    grid=major,
    each nth point={10},
    legend pos={south east},
    legend style={/tikz/every node/.append style={anchor=west}},
    every axis plot/.append style={line width=1pt},
    cycle list name=mycolors,
     title={ELD, N-HiTS},
  ]
  \addplot [gray, dashed, domain=1e-4:1, samples=100, forget plot] {x};
  
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/LiRA/NHiTS-offline/total/roc_MAELoss.csv};
    \addlegendentry{MAE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/LiRA/NHiTS-offline/total/roc_MSELoss.csv};
    \addlegendentry{MSE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/LiRA/NHiTS-offline/total/roc_SeasonalityLoss.csv};
    \addlegendentry{Seasonality}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/LiRA/NHiTS-offline/total/roc_SMAPELoss.csv};
    \addlegendentry{SMAPE Loss}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/LiRA/NHiTS-offline/total/roc_RescaledSMAPELoss.csv};
    \addlegendentry{Rescaled SMAPE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/LiRA/NHiTS-offline/total/roc_TrendLoss.csv};
    \addlegendentry{Trend}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/LiRA/NHiTS-offline/total/roc_TS2VecLoss.csv};
    \addlegendentry{TS2Vec}
  \end{axis}
\end{tikzpicture}
% \caption{Model 1}
\end{subfigure}



==> Results_includes/offline_ROCs_rows/Multi-LiRA.tex <==
\pgfplotsset{
  every axis/.append style={
    label style={font=\normalsize},
    tick label style={font=\normalsize},
    legend style={font=\normalsize},
  }
}

% ------------ Subfigure 1 ------------
\begin{subfigure}[t]{0.22\textwidth}
\centering
\begin{tikzpicture}[scale=0.5]
  \begin{axis}[
    xmode=log, ymode=log,
    log basis y = 10,
    each nth point={10},
    xmin=1e-4, ymin=1e-4, xmax=1, ymax=1,
    xlabel={FPR}, ylabel={TPR (Multi-Signal LiRA)},
    grid=major,
    legend pos={south east},
    legend style={/tikz/every node/.append style={anchor=west}},
    every axis plot/.append style={line width=1pt},
    cycle list name=mycolors,
  ]
    
    \addplot [gray, dashed, domain=1e-4:1, samples=100, forget plot] {x};


    \addplot+[
    mark=none]
    table[x=fpr, y=tpr, col sep=comma] {data/EEG/Multi-LiRA/LSTM-offline/total/roc.csv};
    \addlegendentry{Multi-Signal}
    
  \end{axis}
\end{tikzpicture}
% % % \caption{Model 1}
\end{subfigure}
% ------------ Subfigure 2 ------------
\begin{subfigure}[t]{0.22\textwidth}
\centering
\begin{tikzpicture}[scale=0.5]
  \begin{axis}[
    xmode=log, ymode=log,
    xmin=1e-4, ymin=1e-4, xmax=1, ymax=1,
    xlabel={FPR}, ylabel={},
    grid=major,
    each nth point={10},
    legend pos={south east},
    legend style={/tikz/every node/.append style={anchor=west}},
    every axis plot/.append style={line width=1pt},
    cycle list name=mycolors,
  ]
  \addplot [gray, dashed, domain=1e-4:1, samples=100, forget plot] {x};
  
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/Multi-LiRA/NHiTS-offline/total/roc.csv};
    \addlegendentry{Multi-Signal}
    
  \end{axis}
\end{tikzpicture}
% \caption{Model 2}
\end{subfigure}
% ------------ Subfigure 3 ------------
\begin{subfigure}[t]{0.22\textwidth}
\centering
\begin{tikzpicture}[scale=0.5]
  \begin{axis}[
    xmode=log, ymode=log,
    xmin=1e-4, ymin=1e-4, xmax=1, ymax=1,
    xlabel={FPR}, ylabel={},
    grid=major,
    each nth point={10},
    legend pos={south east},
    legend style={/tikz/every node/.append style={anchor=west}},
    every axis plot/.append style={line width=1pt},
    cycle list name=mycolors,
  ]
  \addplot [gray, dashed, domain=1e-4:1, samples=100, forget plot] {x};
  
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/Multi-LiRA/LSTM-offline/total/roc.csv};
    \addlegendentry{Multi-Signal}
  \end{axis}
\end{tikzpicture}
% % \caption{Model 1}
\end{subfigure}
% ------------ Subfigure 4 ------------
\begin{subfigure}[t]{0.22\textwidth}
\centering
\begin{tikzpicture}[scale=0.5]
  \begin{axis}[
    xmode=log, ymode=log,
    xmin=1e-4, ymin=1e-4, xmax=1, ymax=1,
    xlabel={FPR}, ylabel={},
    grid=major,
    each nth point={10},
    legend pos={south east},
    legend style={/tikz/every node/.append style={anchor=west}},
    every axis plot/.append style={line width=1pt},
    cycle list name=mycolors,
  ]
  \addplot [gray, dashed, domain=1e-4:1, samples=100, forget plot] {x};
  
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/Multi-LiRA/NHiTS-offline/total/roc.csv};
    \addlegendentry{Multi-Signal}
    
  \end{axis}
\end{tikzpicture}
% % \caption{Model 1}
\end{subfigure}


==> Results_includes/offline_ROCs_rows/RMIA.tex <==
\pgfplotsset{
  every axis/.append style={
    label style={font=\normalsize},
    tick label style={font=\normalsize},
    legend style={font=\normalsize},
  }
}

% ------------ Subfigure 1 ------------
\begin{subfigure}[t]{0.22\textwidth}
\centering
\begin{tikzpicture}[scale=0.5]
  \begin{axis}[
    xmode=log, ymode=log,
    log basis y = 10,
    each nth point={10},
    xmin=1e-4, ymin=1e-4, xmax=1, ymax=1,
    xlabel={FPR}, ylabel={TPR (RMIA)},
    grid=major,
    legend pos={south east},
    legend style={/tikz/every node/.append style={anchor=west}},
    every axis plot/.append style={line width=1pt},
    cycle list name=mycolors,
  ]
    
    \addplot [gray, dashed, domain=1e-4:1, samples=100, forget plot] {x};


    \addplot+[
    mark=none]
    table[x=fpr, y=tpr, col sep=comma] {data/EEG/RMIA/LSTM-offline/total/roc_MAELoss.csv};
    \addlegendentry{MAE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/RMIA/LSTM-offline/total/roc_MSELoss.csv};
    \addlegendentry{MSE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/RMIA/LSTM-offline/total/roc_SeasonalityLoss.csv};
    \addlegendentry{Seasonality}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/RMIA/LSTM-offline/total/roc_SMAPELoss.csv};
    \addlegendentry{SMAPE Loss}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/RMIA/LSTM-offline/total/roc_TrendLoss.csv};
    \addlegendentry{Trend}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/RMIA/LSTM-offline/total/roc_TS2VecLoss.csv};
    \addlegendentry{TS2Vec}
    
  \end{axis}
\end{tikzpicture}
% % \caption{Model 1}
\end{subfigure}
% ------------ Subfigure 2 ------------
\begin{subfigure}[t]{0.22\textwidth}
\centering
\begin{tikzpicture}[scale=0.5]
  \begin{axis}[
    xmode=log, ymode=log,
    xmin=1e-4, ymin=1e-4, xmax=1, ymax=1,
    xlabel={FPR}, ylabel={},
    grid=major,
    each nth point={10},
    legend pos={south east},
    legend style={/tikz/every node/.append style={anchor=west}},
    every axis plot/.append style={line width=1pt},
    cycle list name=mycolors,
  ]
  \addplot [gray, dashed, domain=1e-4:1, samples=100, forget plot] {x};
  
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/RMIA/NHiTS-offline/total/roc_MAELoss.csv};
    \addlegendentry{MAE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/RMIA/NHiTS-offline/total/roc_MSELoss.csv};
    \addlegendentry{MSE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/RMIA/NHiTS-offline/total/roc_SeasonalityLoss.csv};
    \addlegendentry{Seasonality}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/RMIA/NHiTS-offline/total/roc_SMAPELoss.csv};
    \addlegendentry{SMAPE Loss}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/RMIA/NHiTS-offline/total/roc_TrendLoss.csv};
    \addlegendentry{Trend}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/RMIA/NHiTS-offline/total/roc_TS2VecLoss.csv};
    \addlegendentry{TS2Vec}
  \end{axis}
\end{tikzpicture}
% \caption{Model 2}
\end{subfigure}
% ------------ Subfigure 3 ------------
\begin{subfigure}[t]{0.22\textwidth}
\centering
\begin{tikzpicture}[scale=0.5]
  \begin{axis}[
    xmode=log, ymode=log,
    xmin=1e-4, ymin=1e-4, xmax=1, ymax=1,
    xlabel={FPR}, ylabel={},
    grid=major,
    each nth point={10},
    legend pos={south east},
    legend style={/tikz/every node/.append style={anchor=west}},
    every axis plot/.append style={line width=1pt},
    cycle list name=mycolors,
  ]
  \addplot [gray, dashed, domain=1e-4:1, samples=100, forget plot] {x};
  
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/RMIA/LSTM-offline/total/roc_MAELoss.csv};
    \addlegendentry{MAE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/RMIA/LSTM-offline/total/roc_MSELoss.csv};
    \addlegendentry{MSE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/RMIA/LSTM-offline/total/roc_SeasonalityLoss.csv};
    \addlegendentry{Seasonality}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/RMIA/LSTM-offline/total/roc_SMAPELoss.csv};
    \addlegendentry{SMAPE Loss}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/RMIA/LSTM-offline/total/roc_TrendLoss.csv};
    \addlegendentry{Trend}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/RMIA/LSTM-offline/total/roc_TS2VecLoss.csv};
    \addlegendentry{TS2Vec}
  \end{axis}
\end{tikzpicture}
% % \caption{Model 1}
\end{subfigure}
% ------------ Subfigure 4 ------------
\begin{subfigure}[t]{0.22\textwidth}
\centering
\begin{tikzpicture}[scale=0.5]
  \begin{axis}[
    xmode=log, ymode=log,
    xmin=1e-4, ymin=1e-4, xmax=1, ymax=1,
    xlabel={FPR}, ylabel={},
    grid=major,
    each nth point={10},
    legend pos={south east},
    legend style={/tikz/every node/.append style={anchor=west}},
    every axis plot/.append style={line width=1pt},
    cycle list name=mycolors,
  ]
  \addplot [gray, dashed, domain=1e-4:1, samples=100, forget plot] {x};
  
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/RMIA/NHiTS-offline/total/roc_MAELoss.csv};
    \addlegendentry{MAE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/RMIA/NHiTS-offline/total/roc_MSELoss.csv};
    \addlegendentry{MSE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/RMIA/NHiTS-offline/total/roc_SeasonalityLoss.csv};
    \addlegendentry{Seasonality}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/RMIA/NHiTS-offline/total/roc_SMAPELoss.csv};
    \addlegendentry{SMAPE Loss}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/RMIA/NHiTS-offline/total/roc_TrendLoss.csv};
    \addlegendentry{Trend}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/RMIA/NHiTS-offline/total/roc_TS2VecLoss.csv};
    \addlegendentry{TS2Vec}
  \end{axis}
\end{tikzpicture}
% % \caption{Model 1}
\end{subfigure}


==> Results_includes/online_ROCs_rows/DTS.tex <==
\pgfplotsset{
  every axis/.append style={
    label style={font=\normalsize},
    tick label style={font=\normalsize},
    legend style={font=\normalsize},
  }
}

% ------------ Subfigure 1 ------------
\begin{subfigure}[t]{0.22\textwidth}
\centering
\begin{tikzpicture}[scale=0.5]
  \begin{axis}[
    xmode=log, ymode=log,
    log basis y = 10,
    each nth point={10},
    xmin=1e-4, ymin=1e-4, xmax=1, ymax=1,
    xlabel={FPR}, ylabel={TPR (DTS)},
    grid=major,
    legend pos={south east},
    legend style={/tikz/every node/.append style={anchor=west}},
    every axis plot/.append style={line width=1pt},
    cycle list name=mycolors,
  ]
    
    \addplot [gray, dashed, domain=1e-4:1, samples=100, forget plot] {x};


    \addplot+[
    mark=none]
    table[x=fpr, y=tpr, col sep=comma] {data/EEG/DTS/LSTM-online/total/roc_InceptionTimeS.csv};
    \addlegendentry{InceptionTime}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/DTS/LSTM-online/total/roc_LSTM.csv};
    \addlegendentry{LSTM}
    
    
  \end{axis}
\end{tikzpicture}
% % \caption{Model 1}
\end{subfigure}
% ------------ Subfigure 2 ------------
\begin{subfigure}[t]{0.22\textwidth}
\centering
\begin{tikzpicture}[scale=0.5]
  \begin{axis}[
    xmode=log, ymode=log,
    xmin=1e-4, ymin=1e-4, xmax=1, ymax=1,
    xlabel={FPR}, ylabel={},
    grid=major,
    each nth point={10},
    legend pos={south east},
    legend style={/tikz/every node/.append style={anchor=west}},
    every axis plot/.append style={line width=1pt},
    cycle list name=mycolors,
  ]
  \addplot [gray, dashed, domain=1e-4:1, samples=100, forget plot] {x};
  
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/DTS/NHiTS-online/total/roc_InceptionTimeS.csv};
    \addlegendentry{InceptionTime}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/DTS/NHiTS-online/total/roc_LSTM.csv};
    \addlegendentry{LSTM}
    
  \end{axis}
\end{tikzpicture}
% \caption{Model 2}
\end{subfigure}
% ------------ Subfigure 3 ------------
\begin{subfigure}[t]{0.22\textwidth}
\centering
\begin{tikzpicture}[scale=0.5]
  \begin{axis}[
    xmode=log, ymode=log,
    xmin=1e-4, ymin=1e-4, xmax=1, ymax=1,
    xlabel={FPR}, ylabel={},
    grid=major,
    each nth point={10},
    legend pos={south east},
    legend style={/tikz/every node/.append style={anchor=west}},
    every axis plot/.append style={line width=1pt},
    cycle list name=mycolors,
  ]
  \addplot [gray, dashed, domain=1e-4:1, samples=100, forget plot] {x};
  
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/DTS/LSTM-online/total/roc_InceptionTimeS.csv};
    \addlegendentry{InceptionTime}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/DTS/LSTM-online/total/roc_LSTM.csv};
    \addlegendentry{LSTM}
    
  \end{axis}
\end{tikzpicture}
% \caption{Model 1}
\end{subfigure}
% ------------ Subfigure 4 ------------
\begin{subfigure}[t]{0.22\textwidth}
\centering
\begin{tikzpicture}[scale=0.5]
  \begin{axis}[
    xmode=log, ymode=log,
    xmin=1e-4, ymin=1e-4, xmax=1, ymax=1,
    xlabel={FPR}, ylabel={},
    grid=major,
    each nth point={10},
    legend pos={south east},
    legend style={/tikz/every node/.append style={anchor=west}},
    every axis plot/.append style={line width=1pt},
    cycle list name=mycolors,
  ]
  \addplot [gray, dashed, domain=1e-4:1, samples=100, forget plot] {x};
  
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/DTS/NHiTS-online/total/roc_InceptionTimeS.csv};
    \addlegendentry{InceptionTime}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/DTS/NHiTS-online/total/roc_LSTM.csv};
    \addlegendentry{LSTM}

  \end{axis}
\end{tikzpicture}
% \caption{Model 1}
\end{subfigure}


==> Results_includes/online_ROCs_rows/Ensemble.tex <==
\pgfplotsset{
  every axis/.append style={
    label style={font=\normalsize},
    tick label style={font=\normalsize},
    legend style={font=\normalsize},
    legend pos={south east},
  }
}

% ------------ Subfigure 1 ------------
\begin{subfigure}[t]{0.22\textwidth}
\centering
\begin{tikzpicture}[scale=0.5]
  \begin{axis}[
    xlabel={FPR}, ylabel={TPR (Ensemble)},
    title={TUH-EEG, LSTM},
    each nth point={5},    % use your variable
    xmode=log,
    ymode=log,
    xmin=1e-4, xmax=1,
    ymin=1e-4, ymax=1,
    grid=major,
    every axis plot/.append style={line width=1pt},
    cycle list name=mycolors
  ]
    
    \addplot [gray, dashed, domain=1e-4:1,samples=200, forget plot] {x};


    \addplot+[
    mark=none]
    table[x=fpr, y=tpr, col sep=comma] {data/EEG/Ensemble/LSTM-audit_mode/total/roc_MAELoss.csv};
    \addlegendentry{MAE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/Ensemble/LSTM-audit_mode/total/roc_MSELoss.csv};
    \addlegendentry{MSE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/Ensemble/LSTM-audit_mode/total/roc_SeasonalityLoss.csv};
    \addlegendentry{Seasonality}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/Ensemble/LSTM-audit_mode/total/roc_SMAPELoss.csv};
    \addlegendentry{SMAPE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/Ensemble/LSTM-audit_mode/total/roc_RescaledSMAPELoss.csv};
    \addlegendentry{rSMAPE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/Ensemble/LSTM-audit_mode/total/roc_TrendLoss.csv};
    \addlegendentry{Trend}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/Ensemble/LSTM-audit_mode/total/roc_TS2VecLoss.csv};
    \addlegendentry{TS2Vec}
    
  \end{axis}
\end{tikzpicture}
% % \caption{Model 1}
\end{subfigure}
% ------------ Subfigure 2 ------------
\begin{subfigure}[t]{0.22\textwidth}
\centering
\begin{tikzpicture}[scale=0.5]
  \begin{axis}[
    xlabel={FPR}, ylabel={},
    title={TUH-EEG, N-HiTS},
    each nth point={5},    % use your variable
    xmode=log,
    ymode=log,
    xmin=1e-4, xmax=1,
    ymin=1e-4, ymax=1,
    grid=major,
    every axis plot/.append style={line width=1pt},
    cycle list name=mycolors
  ]
  \addplot [gray, dashed, domain=1e-4:1, samples=200, forget plot] {x};
  
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/Ensemble/NHiTS-audit_mode/total/roc_MAELoss.csv};
    \addlegendentry{MAE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/Ensemble/NHiTS-audit_mode/total/roc_MSELoss.csv};
    \addlegendentry{MSE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/Ensemble/NHiTS-audit_mode/total/roc_SeasonalityLoss.csv};
    \addlegendentry{Seasonality}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/Ensemble/NHiTS-audit_mode/total/roc_SMAPELoss.csv};
    \addlegendentry{SMAPE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/Ensemble/NHiTS-audit_mode/total/roc_RescaledSMAPELoss.csv};
    \addlegendentry{rSMAPE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/Ensemble/NHiTS-audit_mode/total/roc_TrendLoss.csv};
    \addlegendentry{Trend}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/Ensemble/NHiTS-audit_mode/total/roc_TS2VecLoss.csv};
    \addlegendentry{TS2Vec}
  \end{axis}
\end{tikzpicture}
% \caption{Model 2}
\end{subfigure}
% ------------ Subfigure 3 ------------
\begin{subfigure}[t]{0.22\textwidth}
\centering
\begin{tikzpicture}[scale=0.5]
  \begin{axis}[
    xlabel={FPR}, ylabel={},
    title={ELD, LSTM},
        each nth point={5},    % use your variable
    xmode=log,
    ymode=log,
    xmin=1e-4, xmax=1,
    ymin=1e-4, ymax=1,
    grid=major,
    every axis plot/.append style={line width=1pt},
    cycle list name=mycolors
  ]
  \addplot [gray, dashed, domain=1e-4:1, samples=200, forget plot] {x};
  
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/Ensemble/LSTM-audit_mode/total/roc_MAELoss.csv};
    \addlegendentry{MAE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/Ensemble/LSTM-audit_mode/total/roc_MSELoss.csv};
    \addlegendentry{MSE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/Ensemble/LSTM-audit_mode/total/roc_SeasonalityLoss.csv};
    \addlegendentry{Seasonality}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/Ensemble/LSTM-audit_mode/total/roc_SMAPELoss.csv};
    \addlegendentry{SMAPE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/Ensemble/LSTM-audit_mode/total/roc_RescaledSMAPELoss.csv};
    \addlegendentry{rSMAPE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/Ensemble/LSTM-audit_mode/total/roc_TrendLoss.csv};
    \addlegendentry{Trend}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/Ensemble/LSTM-audit_mode/total/roc_TS2VecLoss.csv};
    \addlegendentry{TS2Vec}
  \end{axis}
\end{tikzpicture}
% \caption{Model 1}
\end{subfigure}
% ------------ Subfigure 5 ------------
\begin{subfigure}[t]{0.22\textwidth}
\centering
\begin{tikzpicture}[scale=0.5]
  \begin{axis}[
    xlabel={FPR}, ylabel={},
    title={ELD, N-HiTS},
        each nth point={5},    % use your variable
    xmode=log,
    ymode=log,
    xmin=1e-4, xmax=1,
    ymin=1e-4, ymax=1,
    grid=major,
    every axis plot/.append style={line width=1pt},
    cycle list name=mycolors
  ]
  \addplot [gray, dashed, domain=1e-4:1, samples=200, forget plot] {x};
  
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/Ensemble/NHiTS-audit_mode/total/roc_MAELoss.csv};
    \addlegendentry{MAE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/Ensemble/NHiTS-audit_mode/total/roc_MSELoss.csv};
    \addlegendentry{MSE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/Ensemble/NHiTS-audit_mode/total/roc_SeasonalityLoss.csv};
    \addlegendentry{Seasonality}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/Ensemble/NHiTS-audit_mode/total/roc_SMAPELoss.csv};
    \addlegendentry{SMAPE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/Ensemble/NHiTS-audit_mode/total/roc_RescaledSMAPELoss.csv};
    \addlegendentry{rSMAPE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/Ensemble/NHiTS-audit_mode/total/roc_TrendLoss.csv};
    \addlegendentry{Trend}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/Ensemble/NHiTS-audit_mode/total/roc_TS2VecLoss.csv};
    \addlegendentry{TS2Vec}
  \end{axis}
\end{tikzpicture}
% \caption{Model 1}
\end{subfigure}


==> Results_includes/online_ROCs_rows/LiRA.tex <==
\pgfplotsset{
  every axis/.append style={
    label style={font=\normalsize},
    tick label style={font=\normalsize},
    legend style={font=\normalsize},
  }
}

% ------------ Subfigure 1 ------------
\begin{subfigure}[t]{0.22\textwidth}
\centering
\begin{tikzpicture}[scale=0.5]
  \begin{axis}[
    xmode=log, ymode=log,
    log basis y = 10,
    each nth point={10},
    xmin=1e-4, ymin=1e-4, xmax=1, ymax=1,
    xlabel={FPR}, ylabel={TPR (LiRA)},
    title={},
    grid=major,
    legend pos={south east},
    legend style={/tikz/every node/.append style={anchor=west}},
    every axis plot/.append style={line width=1pt},
    cycle list name=mycolors,
  ]    
    \addplot [gray, dashed, domain=1e-4:1, samples=100, forget plot] {x};

    \addplot+[
    mark=none]
    table[x=fpr, y=tpr, col sep=comma] {data/EEG/LiRA/LSTM-online/total/roc_MAELoss.csv};
    \addlegendentry{MAE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/LiRA/LSTM-online/total/roc_MSELoss.csv};
    \addlegendentry{MSE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/LiRA/LSTM-online/total/roc_SeasonalityLoss.csv};
    \addlegendentry{Seasonality}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/LiRA/LSTM-online/total/roc_SMAPELoss.csv};
    \addlegendentry{SMAPE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/LiRA/LSTM-online/total/roc_RescaledSMAPELoss.csv};
    \addlegendentry{rSMAPE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/LiRA/LSTM-online/total/roc_TrendLoss.csv};
    \addlegendentry{Trend}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/LiRA/LSTM-online/total/roc_TS2VecLoss.csv};
    \addlegendentry{TS2Vec}
    
  \end{axis}
\end{tikzpicture}
% \caption{Model 1}
\end{subfigure}
% ------------ Subfigure 2 ------------
\begin{subfigure}[t]{0.22\textwidth}
\centering
\begin{tikzpicture}[scale=0.5]
  \begin{axis}[
    xmode=log, ymode=log,
    xmin=1e-4, ymin=1e-4, xmax=1, ymax=1,
    xlabel={FPR}, ylabel={},
    grid=major,
    each nth point={10},
    legend pos={south east},
    legend style={/tikz/every node/.append style={anchor=west}},
    every axis plot/.append style={line width=1pt},
    cycle list name=mycolors,
  ]
  \addplot [gray, dashed, domain=1e-4:1, samples=100, forget plot] {x};
  
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/LiRA/NHiTS-online/total/roc_MAELoss.csv};
    \addlegendentry{MAE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/LiRA/NHiTS-online/total/roc_MSELoss.csv};
    \addlegendentry{MSE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/LiRA/NHiTS-online/total/roc_SeasonalityLoss.csv};
    \addlegendentry{Seasonality}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/LiRA/NHiTS-online/total/roc_SMAPELoss.csv};
    \addlegendentry{SMAPE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/LiRA/NHiTS-online/total/roc_RescaledSMAPELoss.csv};
    \addlegendentry{rSMAPE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/LiRA/NHiTS-online/total/roc_TrendLoss.csv};
    \addlegendentry{Trend}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/LiRA/NHiTS-online/total/roc_TS2VecLoss.csv};
    \addlegendentry{TS2Vec}
  \end{axis}
\end{tikzpicture}
% \caption{Model 2}
\end{subfigure}
% ------------ Subfigure 3 ------------
\begin{subfigure}[t]{0.22\textwidth}
\centering
\begin{tikzpicture}[scale=0.5]
  \begin{axis}[
    xmode=log, ymode=log,
    xmin=1e-4, ymin=1e-4, xmax=1, ymax=1,
    xlabel={FPR}, ylabel={},
    grid=major,
    each nth point={10},
    legend pos={south east},
    legend style={/tikz/every node/.append style={anchor=west}},
    every axis plot/.append style={line width=1pt},
    cycle list name=mycolors,
  ]
  \addplot [gray, dashed, domain=1e-4:1, samples=100, forget plot] {x};
  
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/LiRA/LSTM-online/total/roc_MAELoss.csv};
    \addlegendentry{MAE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/LiRA/LSTM-online/total/roc_MSELoss.csv};
    \addlegendentry{MSE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/LiRA/LSTM-online/total/roc_SeasonalityLoss.csv};
    \addlegendentry{Seasonality}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/LiRA/LSTM-online/total/roc_SMAPELoss.csv};
    \addlegendentry{SMAPE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/LiRA/LSTM-online/total/roc_RescaledSMAPELoss.csv};
    \addlegendentry{rSMAPE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/LiRA/LSTM-online/total/roc_TrendLoss.csv};
    \addlegendentry{Trend}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/LiRA/LSTM-online/total/roc_TS2VecLoss.csv};
    \addlegendentry{TS2Vec}
  \end{axis}
\end{tikzpicture}
% \caption{Model 1}
\end{subfigure}
% ------------ Subfigure 4 ------------
\begin{subfigure}[t]{0.22\textwidth}
\centering
\begin{tikzpicture}[scale=0.5]
  \begin{axis}[
    xmode=log, ymode=log,
    xmin=1e-4, ymin=1e-4, xmax=1, ymax=1,
    xlabel={FPR}, ylabel={},
    grid=major,
    each nth point={10},
    legend pos={south east},
    legend style={/tikz/every node/.append style={anchor=west}},
    every axis plot/.append style={line width=1pt},
    cycle list name=mycolors,
  ]
  \addplot [gray, dashed, domain=1e-4:1, samples=100, forget plot] {x};
  
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/LiRA/NHiTS-online/total/roc_MAELoss.csv};
    \addlegendentry{MAE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/LiRA/NHiTS-online/total/roc_MSELoss.csv};
    \addlegendentry{MSE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/LiRA/NHiTS-online/total/roc_SeasonalityLoss.csv};
    \addlegendentry{Seasonality}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/LiRA/NHiTS-online/total/roc_SMAPELoss.csv};
    \addlegendentry{SMAPE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/LiRA/NHiTS-online/total/roc_RescaledSMAPELoss.csv};
    \addlegendentry{rSMAPE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/LiRA/NHiTS-online/total/roc_TrendLoss.csv};
    \addlegendentry{Trend}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/LiRA/NHiTS-online/total/roc_TS2VecLoss.csv};
    \addlegendentry{TS2Vec}
  \end{axis}
\end{tikzpicture}
% \caption{Model 1}
\end{subfigure}



==> Results_includes/online_ROCs_rows/Multi-LiRA.tex <==
\pgfplotsset{
  every axis/.append style={
    label style={font=\normalsize},
    tick label style={font=\normalsize},
    legend style={font=\normalsize},
  }
}

% ------------ Subfigure 1 ------------
\begin{subfigure}[t]{0.22\textwidth}
\centering
\begin{tikzpicture}[scale=0.5]
  \begin{axis}[
    xmode=log, ymode=log,
    log basis y = 10,
    each nth point={10},
    xmin=1e-4, ymin=1e-4, xmax=1, ymax=1,
    xlabel={FPR}, ylabel={TPR (Multi-Signal LiRA)},
    grid=major,
    legend pos={south east},
    legend style={/tikz/every node/.append style={anchor=west}},
    every axis plot/.append style={line width=1pt},
    cycle list name=mycolors,
  ]

    \addplot [gray, dashed, domain=1e-4:1, samples=100, forget plot] {x};

    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/Multi-LiRA/LSTM-online/total/roc.csv};
    \addlegendentry{Multi-Signal}
    
  \end{axis}
\end{tikzpicture}
% % % \caption{Model 1}
\end{subfigure}
% ------------ Subfigure 2 ------------
\begin{subfigure}[t]{0.22\textwidth}
\centering
\begin{tikzpicture}[scale=0.5]
  \begin{axis}[
    xmode=log, ymode=log,
    xmin=1e-4, ymin=1e-4, xmax=1, ymax=1,
    xlabel={FPR}, ylabel={},
    grid=major,
    each nth point={10},
    legend pos={south east},
    legend style={/tikz/every node/.append style={anchor=west}},
    every axis plot/.append style={line width=1pt},
    cycle list name=mycolors,
  ]
  \addplot [gray, dashed, domain=1e-4:1, samples=100, forget plot] {x};
  
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/Multi-LiRA/NHiTS-online/total/roc.csv};
    \addlegendentry{Multi-Signal}
    
  \end{axis}
\end{tikzpicture}
% \caption{Model 2}
\end{subfigure}
% ------------ Subfigure 3 ------------
\begin{subfigure}[t]{0.22\textwidth}
\centering
\begin{tikzpicture}[scale=0.5]
  \begin{axis}[
    xmode=log, ymode=log,
    xmin=1e-4, ymin=1e-4, xmax=1, ymax=1,
    xlabel={FPR}, ylabel={},
    grid=major,
    each nth point={10},
    legend pos={south east},
    legend style={/tikz/every node/.append style={anchor=west}},
    every axis plot/.append style={line width=1pt},
    cycle list name=mycolors,
  ]
  \addplot [gray, dashed, domain=1e-4:1, samples=100, forget plot] {x};
  
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/Multi-LiRA/LSTM-online/total/roc.csv};
    \addlegendentry{Multi-Signal}
  \end{axis}
\end{tikzpicture}
% % \caption{Model 1}
\end{subfigure}
% ------------ Subfigure 4 ------------
\begin{subfigure}[t]{0.22\textwidth}
\centering
\begin{tikzpicture}[scale=0.5]
  \begin{axis}[
    xmode=log, ymode=log,
    xmin=1e-4, ymin=1e-4, xmax=1, ymax=1,
    xlabel={FPR}, ylabel={},
    grid=major,
    each nth point={10},
    legend pos={south east},
    legend style={/tikz/every node/.append style={anchor=west}},
    every axis plot/.append style={line width=1pt},
    cycle list name=mycolors,
  ]
  \addplot [gray, dashed, domain=1e-4:1, samples=100, forget plot] {x};
  
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/Multi-LiRA/NHiTS-online/total/roc.csv};
    \addlegendentry{Multi-Signal}
    
  \end{axis}
\end{tikzpicture}
% % \caption{Model 1}
\end{subfigure}


==> Results_includes/online_ROCs_rows/RMIA.tex <==
\pgfplotsset{
  every axis/.append style={
    label style={font=\normalsize},
    tick label style={font=\normalsize},
    legend style={font=\normalsize},
  },
}

% ------------ Subfigure 1 ------------
\begin{subfigure}[t]{0.22\textwidth}
\centering
\begin{tikzpicture}[scale=0.5]
  \begin{axis}[
    xmode=log, ymode=log,
    log basis y = 10,
    each nth point={10},
    xmin=1e-4, ymin=1e-4, xmax=1, ymax=1,
    xlabel={FPR}, ylabel={TPR (RMIA)},
    grid=major,
    legend pos={south east},
    legend style={/tikz/every node/.append style={anchor=west}},
    every axis plot/.append style={line width=1pt},
    cycle list name=mycolors,
  ]
    
    \addplot [gray, dashed, domain=1e-4:1, samples=100, forget plot] {x};


    \addplot+[
    mark=none]
    table[x=fpr, y=tpr, col sep=comma] {data/EEG/RMIA/LSTM-online/total/roc_MAELoss.csv};
    \addlegendentry{MAE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/RMIA/LSTM-online/total/roc_MSELoss.csv};
    \addlegendentry{MSE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/RMIA/LSTM-online/total/roc_SeasonalityLoss.csv};
    \addlegendentry{Seasonality}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/RMIA/LSTM-online/total/roc_SMAPELoss.csv};
    \addlegendentry{SMAPE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/RMIA/LSTM-online/total/roc_TrendLoss.csv};
    \addlegendentry{Trend}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/RMIA/LSTM-online/total/roc_TS2VecLoss.csv};
    \addlegendentry{TS2Vec}
    
  \end{axis}
\end{tikzpicture}
% % \caption{Model 1}
\end{subfigure}
% ------------ Subfigure 2 ------------
\begin{subfigure}[t]{0.22\textwidth}
\centering
\begin{tikzpicture}[scale=0.5]
  \begin{axis}[
    xmode=log, ymode=log,
    xmin=1e-4, ymin=1e-4, xmax=1, ymax=1,
    xlabel={FPR}, ylabel={},
    grid=major,
    each nth point={10},
    legend pos={south east},
    legend style={/tikz/every node/.append style={anchor=west}},
    every axis plot/.append style={line width=1pt},
    cycle list name=mycolors,
  ]
  \addplot [gray, dashed, domain=1e-4:1, samples=100, forget plot] {x};
  
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/RMIA/NHiTS-online/total/roc_MAELoss.csv};
    \addlegendentry{MAE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/RMIA/NHiTS-online/total/roc_MSELoss.csv};
    \addlegendentry{MSE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/RMIA/NHiTS-online/total/roc_SeasonalityLoss.csv};
    \addlegendentry{Seasonality}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/RMIA/NHiTS-online/total/roc_SMAPELoss.csv};
    \addlegendentry{SMAPE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/RMIA/NHiTS-online/total/roc_TrendLoss.csv};
    \addlegendentry{Trend}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/EEG/RMIA/NHiTS-online/total/roc_TS2VecLoss.csv};
    \addlegendentry{TS2Vec}
  \end{axis}
\end{tikzpicture}
% \caption{Model 2}
\end{subfigure}
% ------------ Subfigure 3 ------------
\begin{subfigure}[t]{0.22\textwidth}
\centering
\begin{tikzpicture}[scale=0.5]
  \begin{axis}[
    xmode=log, ymode=log,
    xmin=1e-4, ymin=1e-4, xmax=1, ymax=1,
    xlabel={FPR}, ylabel={},
    grid=major,
    each nth point={10},
    legend pos={south east},
    legend style={/tikz/every node/.append style={anchor=west}},
    every axis plot/.append style={line width=1pt},
    cycle list name=mycolors,
  ]
  \addplot [gray, dashed, domain=1e-4:1, samples=100, forget plot] {x};
  
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/RMIA/LSTM-online/total/roc_MAELoss.csv};
    \addlegendentry{MAE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/RMIA/LSTM-online/total/roc_MSELoss.csv};
    \addlegendentry{MSE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/RMIA/LSTM-online/total/roc_SeasonalityLoss.csv};
    \addlegendentry{Seasonality}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/RMIA/LSTM-online/total/roc_SMAPELoss.csv};
    \addlegendentry{SMAPE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/RMIA/LSTM-online/total/roc_TrendLoss.csv};
    \addlegendentry{Trend}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/RMIA/LSTM-online/total/roc_TS2VecLoss.csv};
    \addlegendentry{TS2Vec}
  \end{axis}
\end{tikzpicture}
% % \caption{Model 1}
\end{subfigure}
% ------------ Subfigure 4 ------------
\begin{subfigure}[t]{0.22\textwidth}
\centering
\begin{tikzpicture}[scale=0.5]
  \begin{axis}[
    xmode=log, ymode=log,
    xmin=1e-4, ymin=1e-4, xmax=1, ymax=1,
    xlabel={FPR}, ylabel={},
    grid=major,
    each nth point={10},
    legend pos={south east},
    legend style={/tikz/every node/.append style={anchor=west}},
    every axis plot/.append style={line width=1pt},
    cycle list name=mycolors,
  ]
  \addplot [gray, dashed, domain=1e-4:1, samples=100, forget plot] {x};
  
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/RMIA/NHiTS-online/total/roc_MAELoss.csv};
    \addlegendentry{MAE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/RMIA/NHiTS-online/total/roc_MSELoss.csv};
    \addlegendentry{MSE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/RMIA/NHiTS-online/total/roc_SeasonalityLoss.csv};
    \addlegendentry{Seasonality}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/RMIA/NHiTS-online/total/roc_SMAPELoss.csv};
    \addlegendentry{SMAPE}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/RMIA/NHiTS-online/total/roc_TrendLoss.csv};
    \addlegendentry{Trend}
    
    \addplot+[mark=none]
      table[x=fpr, y=tpr, col sep=comma] {data/ELD/RMIA/NHiTS-online/total/roc_TS2VecLoss.csv};
    \addlegendentry{TS2Vec}
  \end{axis}
\end{tikzpicture}
% % \caption{Model 1}
\end{subfigure}

